Infinite Determinantal Measures and The Ergodic Decomposition of Infinite Pickrell Measures II. Convergence of determinantal measures

The second part of the paper mainly deals with convergence of infinite determinantal measures, understood as the convergence of the approximating finite determinantal measures. In addition to the usual weak topology on the space of probability measures on the space of configurations, we also consider the weak topology on the space of finite measures on the space of finite measures on the half-line, used via the natural immersion, well-defined almost surely with respect to the infinite Bessel point process, of the space of configurations into the space of finite measures on the half-line. The main results of the second part are sufficient conditions for tightness of families of determinantal measures, for convergence of sequences of induced proceses, as well as for sequences of finite-dimensional perturbations of determinantal processes.

==> extref-arxiv.tex <==
% File for inter-part referencing
%------ Macros

\makeatletter

\newcommand{\newlonglabel}[3]{
\def\@@foo{#2}%
\ifx\thispartnum\@@foo\relax
\@bsphack\protected@write\@auxout{}{\string\checklonglabel{#1}{#3}}\@esphack
\else
\@bsphack\protected@write\@auxout{}{\string\newlabel{#1}{{#2.#3}{--}}}\@esphack
\fi
}
\let\checklonglabel\@gobbletwo

\AtEndDocument{\def\checklonglabel#1#2{{\@ifundefined{r@#1}%
{\GenericWarning{}{Longlabel `#1' of this part has label of the same name undefined}}%
{\edef\@@foox{\expandafter\expandafter\expandafter\@firstoftwo\csname r@#1\endcsname}\def\@@fooy{#2}%
\ifx\@@foox\@@fooy\relax\else
\GenericWarning{}{Longlabel `#1' of this part does not coincide with the label of the same name}%
\fi}}}}

\let\longref=\ref
\makeatother


%------ Part I

\newlonglabel{asympt-R-bessel}{I}{1.3}
\newlonglabel{bs-sing}{I}{1.4}
\newlonglabel{singul}{I}{1.9}
\newlonglabel{mainthm-fin}{I}{1.10}
\newlonglabel{mainthm}{I}{1.11}
\newlonglabel{main-lemma}{I}{1.14}
\newlonglabel{expbetaint}{I}{1.15}
\newlonglabel{weak-pick}{I}{1.16}
\newlonglabel{rad-jac}{I}{1.17}
\newlonglabel{det-CDJ}{I}{5}
\newlonglabel{expaa}{I}{8}
\newlonglabel{pisb}{I}{9}
\newlonglabel{rinftymu}{I}{14}
\newlonglabel{rad-u-coord}{I}{17}

\newlonglabel{infdet-he}{I}{2.11}
\newlonglabel{mult-he1}{I}{2.14}
\newlonglabel{closedsubsp}{I}{2.18}
\newlonglabel{fin-rank-mult}{I}{2.19}
\newlonglabel{lin-ind}{I}{2.21}
\newlonglabel{lve}{I}{3}
\newlonglabel{def-Pi-g}{I}{21}

\newlonglabel{tilde-kernel-kns-js}{I}{A.3}
\newlonglabel{CDJ}{I}{34}

\newlonglabel{fin-distr-unique}{I}{B.1}
\newlonglabel{pr1-bis}{I}{B.3}

\newlonglabel{inf-prod-s}{I}{40}

%------ Part II

\newlonglabel{conv-induced}{II}{2.3}
\newlonglabel{conv-inf-det}{II}{2.6}
\newlonglabel{conv-unif-finrank}{II}{3.13}

%------ Part III

% None

\endinput

